Critical Phenomena in Gravitational Collapse

As first discovered by Choptuik, the black hole threshold in the space of initial data for general relativity shows both surprising structure and surprising simplicity. Universality, power-law scaling of the black hole mass, and scale echoing have given rise to the term ``critical phenomena''. They are explained by the existence of exact solutions which are attractors within the black hole threshold, that is, attractors of codimension one in phase space, and which are typically self-similar. Critical phenomena give a natural route from smooth initial data to arbitrarily large curvatures visible from infinity, and are therefore likely to be relevant for cosmic censorship, quantum gravity, astrophysics, and our general understanding of the dynamics of general relativity. Major additions since the 2010 version of this review are numerical simulations beyond spherical symmetry, in particular of vacuum critical collapse, and new sections on mathematical results in PDE blowup (as a toy model for singularity formation) and on naked singularity formation in GR.

==> README <==
This tarball contains the source for the arXiv submission of the 20205
update of the living review Critical Phenomena in Gravitational
Collapse, by Carsten Gundlach, David Hilditch and Jos\'e
M. Martin-Garcia.

To render a version of the article with the new material highlighted,
open critphen_lrr_header.tex and toggle to the alternative \new
command.
